Cardinality Estimation over Knowledge Graphs with Embeddings and Graph Neural Networks

Cardinality Estimation over Knowledge Graphs (KG) is crucial for query optimization, yet remains a challenging task due to the semi-structured nature and complex correlations of typical Knowledge Graphs. In this work, we propose GNCE, a novel approach that leverages knowledge graph embeddings and Graph Neural Networks (GNN) to accurately predict the cardinality of conjunctive queries. GNCE first creates semantically meaningful embeddings for all entities in the KG, which are then integrated into the given query, which is processed by a GNN to estimate the cardinality of the query. We evaluate GNCE on several KGs in terms of q-Error and demonstrate that it outperforms state-of-the-art approaches based on sampling, summaries, and (machine) learning in terms of estimation accuracy while also having lower execution time and less parameters. Additionally, we show that GNCE can inductively generalise to unseen entities, making it suitable for use in dynamic query processing scenarios. Our proposed approach has the potential to significantly improve query optimization and related applications that rely on accurate cardinality estimates of conjunctive queries.

==> tables/res-qerror-complex.tex <==




% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\caption{Mean q-Errors for complex queries on yago}
\label{q_table_complex}
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textit{Wanderjoin} & \textit{impr} & \textit{jsub} & \textit{CSET} & \textit{SUMRDF} & \textit{LMKG} & \textit{LSS} & \textit{GNCE} \\ \hline
226282 & 508309 & 227163 & $3 \cdot e^{27}$ & - & 113 & 2519 & \textbf{8.4} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/res_inductive.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
  \caption{Difference in Q-Error for star queries of unseen entities with respect to results from Table \ref{q_table_star} on SWDF}
\label{fig:inductive_result}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|r|r|r|r|r|r|r|r|}
\hline
\diagbox{Method}{$||Q||_\mathcal{G}$} & $<5$ & $<5^2$ & $<5^3$ & $<5^4$ & $<5^5$ & $<5^6$ & $<5^9$ \\ \hline
\textit{LMKG} & $\downarrow 0.03$ & $\downarrow \mathbf{0.13}$ & $\downarrow 2.36$ & $\downarrow 26.85$ & $\downarrow 145.42$ & $\downarrow 481.81$ & $\downarrow 944.26$ \\ \hline
\textit{LSS} & $\uparrow \mathbf{0.45}$ & $\downarrow 2.23$ & $\downarrow 11.39$ & $\downarrow 90.81$ & $\downarrow 501.30$ & $\downarrow 2313.09$ & $\downarrow 2441.83$ \\ \hline
\textit{GNCE} & $\downarrow 0.25$ & $\downarrow 0.33$ & $\downarrow \mathbf{0.99}$ & $\downarrow \mathbf{3.76}$ & $\downarrow \mathbf{6.88}$ & $\downarrow \mathbf{22.57}$ & $\downarrow \mathbf{3.01}$ \\ \hline
\end{tabular}%
}
\end{table}


==> tables/res_inductive_yago.tex <==
\begin{table}[]
  \caption{Mean q-Error for full inductive learning on Yago star queries.}
  \label{fig:inductive_result_modified_yago}
  \footnotesize
  \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{|r|r|r|r|r|r|r|r|}
      \hline
      \multicolumn{8}{|c|}{Dataset: YAGO}\\
      \hline
      {||Q||} & GNCE & LMKG & LSS & WJ & impr & jsub & CSET \\ \hline
      \(< 5\) & 189.48 & 319.94 & 8.58 & \textbf{2.51} & \textbf{2.51} & \textbf{2.51} & 12133.80 \\ \hline
      \(< 5^2\) & 229.71 & 138.35 & \textbf{3.94} & 11.60 & 13.55 & 13.55 & 13244.83 \\ \hline
      \(< 5^3\) & 73.98 & 47.19 & \textbf{8.10} & 33.96 & 50.27 & 42.74 & 25952.18 \\ \hline
      \(< 5^4\) & \textbf{38.18} & 145.65 & 41.76 & 185.62 & 262.63 & 218.33 & 13092.83 \\ \hline
      \(< 5^5\) & \textbf{44.89} & 595.18 & 196.23 & 628.17 & 1036.19 & 1012.65 & 64086.77 \\ \hline
      \(< 5^6\) & \textbf{86.65} & 2585.38 & 917.44 & 4249.70 & 6114.76 & 4277.01 & 119876.0 \\ \hline
      \(< 5^9\) & \textbf{280.94} & 49462.4 & 19016.3 & 141838.6 & 171508.1 & 142063.0 & 145802.6 \\ \hline
      Avg & \textbf{134.83} & 7613.44 & 2884.61 & 20992.88 & 25569.72 & 21089.98 & 56312.71 \\ \hline
    \end{tabular}
  }
\end{table}

